Refutation of Shapley Values for XAI -- Additional Evidence

Recent work demonstrated the inadequacy of Shapley values for explainable artificial intelligence (XAI). Although to disprove a theory a single counterexample suffices, a possible criticism of earlier work is that the focus was solely on Boolean classifiers. To address such possible criticism, this paper demonstrates the inadequacy of Shapley values for families of classifiers where features are not boolean, but also for families of classifiers for which multiple classes can be picked. Furthermore, the paper shows that the features changed in any minimal $l_0$ distance adversarial examples do not include irrelevant features, thus offering further arguments regarding the inadequacy of Shapley values for XAI.

==> exampl05old.tex <==

\input{./figs/clssf00}

\section{Another Example for Journal Submission}

Besides~\cref{fig:00}, the rest of the analysis mimics that
of~\cref{fig:02}.


Given the discussion in~\cref{sec:ex07}, we have that,

\begin{align}
  \sv(1)
  =~&\nfrac{\alpha}{2}-\nfrac{(2\sigma_1+2\sigma_2+5\sigma_3+4\sigma_4+4\sigma_5+19\sigma_6)}{72}
  = 0 \label{eq:00:cond01} \\
  \sv(2) =~&\nfrac{(-2\sigma_1-2\sigma_2-5\sigma_3+2\sigma_4+2\sigma_5+5\sigma_6)}{72}
  \not= 0 \label{eq:00:cond02} \\
  \sv(3) =~&\nfrac{(-\sigma_1-\sigma_2+2\sigma_3-2\sigma_4-2\sigma_5+4\sigma_6)}{36}
  \not=0 \label{eq:00:cond03} %%\\
\end{align}

Indeed, with $\alpha=1$, $\sigma_1=\sigma_2=\sigma_3=4$ and
$\sigma_4=\sigma_5=\sigma_6=0$, we have that,
\[
\begin{array}{l}
  \sv(1) = 0 \\
  \sv(2) = -\nfrac{1}{2} \not= 0 \\
  \sv(3) = 0 \quad \tn{(!!)}
\end{array}
\]


==> figs/clssf00.tex <==
\begin{figure*}[t]
  \begin{mdframed}[linewidth=1.5pt,linecolor=darkblue,roundcorner=5pt] %skipabove=10pt
    \begin{subfigure}[b]{0.25\textwidth}
      \input{./texfigs/dt00}
      %\begin{tabular}{c} \\[5pt] \\[5pt] \\[5pt] \end{tabular}
      %%%$\kappa(\cdot) = \ldots$
      \caption{Decision tree (DT) for $\kappa$} \label{fig:00:dt}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.35\textwidth}
      \begin{center}
        \begin{tabular}{cccccc} \toprule
          row \# & $x_1$ & $x_2$ & $x_3$ & $\kappa(\mbf{x})$
          \\ \toprule
          1 & 0 & 0 & 0 & 0 \\
          2 & 0 & 0 & 1 & 4 \\
          3 & 0 & 0 & 2 & 0 \\
          4 & 0 & 1 & 0 & 0 \\
          5 & 0 & 1 & 1 & 7 \\
          6 & 0 & 1 & 2 & 0 \\
          7 & 1 & 0 & 0 & 1 \\
          8 & 1 & 0 & 1 & 1 \\
          9 & 1 & 0 & 2 & 1 \\
          10 & 1 & 1 & 0 & 1 \\
          11 & 1 & 1 & 1 & 1 \\
          12 & 1 & 1 & 2 & 1 \\
          \bottomrule
        \end{tabular}
      \end{center}
      \medskip %%\begin{tabular}{c} \\ \end{tabular}
      \caption{Tabular representation (TR) for $\kappa$} \label{fig:00:tt}
    \end{subfigure}
    %\captionof{figure}{Example classifier -- decision tree} \label{fig:example01}
    %
    \begin{subfigure}[b]{0.35\textwidth}
      \setlength{\fboxrule}{0.875pt}
      \setlength{\fboxsep}{2pt}
      \fbox{
        \begin{minipage}{\textwidth}
          Analysis of the classifier: \\
          %DT \& truth table (TT): \\ %Instance $((1,1,2),1)$: \\
          From the DT/TR, it is clear the prediction is 1 whenever
          $x_1=1$, \emph{independently} of the values of $x_2$ and
          $x_3$. %\\
          Hence, for point $\mbf{v}=(1,1,2)$, the prediction will be 1 as
          long as $x_1=1$, \emph{independently} of $x_2$ and $x_3$.
          To change the prediction, the value of $x_1$ must be
          changed. In this case, the prediction will change,
          \emph{independently} of the values of $x_2$ and $x_3$.\\
          Thus, given the instance $((1,1,2),1)$, the value of the
          prediction is determined \emph{uniquely} by the value of
          $x_1$, and it is independent of the values of $x_2$ and
          $x_3$. A change of prediction is also \emph{uniquely}
          determined by the value of $x_1$, and it is again
          independent of $x_2$ and $x_3$.
        \end{minipage}
      }
      \caption{Influence of features on $\kappa$ for $((1,1,2),1)$}
      \label{fig:00:disc}
    \end{subfigure}

    \caption{Example classifier -- decision tree and its tabular
      representation.
     For this classifier, we have $\fml{F}=\{1,2,3\}$,
     $\mbb{D}_1=\mbb{D}_2=\{0,1\}$, and $\mbb{D}_3=\{0,1,2\}$,
     $\mbb{F}=\{0,1\}^2\times\{0,1,2\}$, and
     $\fml{K}=\{0,1,2,3,4,5,6,7\}$, albeit the DT and TR only use 0, 1,
     4 and 7.
     Literals in the DT are represented with set notation, as proposed
     in earlier work~\cite{iims-jair22}, which yields more compact DTs.
     The classification function is given by the decision tree, or
     alternatively by the tabular representation.
     The instance considered is $((1,1,2),1)$, which is consistent
     with path $\langle1,3\rangle$; this path is highlighted in the
     DT. The prediction is 1, as indicated in terminal node 3.%\\
    }
    \label{fig:00}
  \end{mdframed}
\end{figure*}
    


==> figs/clssf00old.tex <==
\begin{figure*}[t]
  \begin{mdframed}[linewidth=1.5pt,linecolor=darkblue,roundcorner=5pt] %skipabove=10pt
    \begin{subfigure}[b]{0.225\textwidth}
      \input{./texfigs/dt00}
      \begin{tabular}{c} \\[5pt] \\[5pt] \\[5pt] \end{tabular}
      %%%$\kappa(\cdot) = \ldots$
      \caption{Decision tree (DT) for $\kappa$} \label{fig:00:dt}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.3\textwidth}
      \begin{center}
        \begin{tabular}{cccccc} \toprule
          row \# & $x_1$ & $x_2$ & $x_3$ & $\kappa(\mbf{x})$
          \\ \toprule
          1 & 0 & 0 & 0 & 4 \\
          2 & 0 & 0 & 1 & 4 \\
          3 & 0 & 0 & 2 & 4 \\
          4 & 0 & 1 & 0 & 0 \\
          5 & 0 & 1 & 1 & 0 \\
          6 & 0 & 1 & 2 & 0 \\
          7 & 1 & 0 & 0 & 1 \\
          8 & 1 & 0 & 1 & 1 \\
          9 & 1 & 0 & 2 & 1 \\
          10 & 1 & 1 & 0 & 1 \\
          11 & 1 & 1 & 1 & 1 \\
          12 & 1 & 1 & 2 & 1 \\
          \bottomrule
        \end{tabular}
      \end{center}
      %%\begin{tabular}{c} \\ \end{tabular}
      \caption{Tabular representation (TR) for $\kappa$} \label{fig:00:tt}
    \end{subfigure}
    %\captionof{figure}{Example classifier -- decision tree} \label{fig:example01}
    %
    \begin{subfigure}[b]{0.425\textwidth}
      \setlength{\fboxrule}{0.875pt}
      \setlength{\fboxsep}{2pt}
      \fbox{
        \begin{minipage}{\textwidth}
          Analysis of the classifier: \\
          %DT \& truth table (TT): \\ %Instance $((1,1,2),1)$: \\
          From the DT/TR, it is clear the prediction is 1 whenever
          $x_1=1$, \emph{independently} of the values of $x_2$ and
          $x_3$. %\\
          Hence, for point $\mbf{v}=(1,1,2)$, the prediction will be 1 as
          long as $x_1=1$, \emph{independently} of $x_2$ and $x_3$.
          To change the prediction, the value of $x_1$ must be
          changed. In this case, the prediction will change,
          \emph{independently} of the values of $x_2$ and $x_3$.\\
          Thus, given the instance $((1,1,2),1)$, the value of the
          prediction is determined \emph{uniquely} by the value of
          $x_1$, and it is independent of the values of $x_2$ and
          $x_3$. A change of prediction is also \emph{uniquely}
          determined by the value of $x_1$, and it is again
          independent of $x_2$ and $x_3$.
        \end{minipage}
      }
      \caption{Influence of features on $\kappa$ for $((1,1,2),1)$}
      \label{fig:00:disc}
    \end{subfigure}

    \caption{Example classifier -- decision tree and its tabular
      representation.
     For this classifier, we have $\fml{F}=\{1,2,3\}$,
     $\mbb{D}_1=\mbb{D}_2=\{0,1\}$, and $\mbb{D}_3=\{0,1,2\}$,
     $\mbb{F}=\{0,1\}^2\times\{0,1,2\}$, and
     $\fml{K}=\{0,1,2,3,4,5,6\}$, albeit the DT and TR only use 0, 1,
     3 and 6.
     Literals in the DT are represented with set notation, as proposed
     in earlier work~\cite{iims-jair22}, which yields more compact DTs.
     The classification function is given by the decision tree, or
     alternatively by the tabular representation.
     The instance considered is $((1,1,2),1)$, which is consistent
     with path $\langle1,3\rangle$; this path is highlighted in the
     DT. The prediction is 1, as indicated in terminal node 3.%\\
    }
    \label{fig:00}
  \end{mdframed}
\end{figure*}
    


==> res.tex <==

%
\section{Case Studies} \label{sec:results}
%
In this section, we pick two concrete decision tree examples
and analyze whether there are instances exhibit $\irrelevant(i) \land \relevant(j) \land (|\sv(i)| > |\sv(j)|)$.
%
The experiments were performed on a MacBook Pro with a 6-Core Intel
Core i7 2.6 GHz processor with 16 GByte RAM, running macOS Ventura.

\paragraph{Example Decision Trees.}
%
We consider 2 publicly available decision trees with discrete features and classes,
as depicted in~\cref{fig:dt03,fig:dt04}.
\cref{fig:domlgb} shows the feature domains of the DT in~\cref{fig:dt03},
while \cref{fig:domz} shows the feature domains of the DT in~\cref{fig:dt04}.

\input{./figs/dtlgb}

\begin{figure*}[t]
  \input{./texfigs/dt03}
  \caption{Example DT, adapted from~\cite{belmonte-ieee-access20}}
  \label{fig:dt03}
\end{figure*}

\clearpage

\input{./figs/dtz}

\begin{figure*}[t]
  \input{./texfigs/dt04}
  \caption{Example DT, adapted from~\cite{zhou2021machine}}
  \label{fig:dt04}
\end{figure*}

\paragraph{Results.}
%
\begin{figure*}
    \begin{center}
    \subcaptionbox{DT adapted from the~\cite{belmonte-ieee-access20}}{
        \includegraphics[width=.45\textwidth]{./figs/res/LGB-paper20-fig9-dt}
    }
    \subcaptionbox{DT adapted from the~\cite{zhou2021machine}}{
        \includegraphics[width=.45\textwidth]{./figs/res/Z21-fig48}
    }
    \caption{
    Whether there exist irrelevant features (dots in yellow) with higher scores than relevant features (dots in blue) in absolute value.}
    \label{fig:shap_scores}
    \end{center}
\end{figure*}

For each instance, all AXps are enumerated to decide which features are relevant and which are irrelevant.
Then we compute Sv for each feature and analyze whether the issue $\irrelevant(i) \land \relevant(j) \land (|\sv(i)| > |\sv(j)|)$ occurs.
%
If an instance exhibits such an issue, we plot a pair of values $(v_i, v_j)$.
More specifically, $v_i = \max\{|\sv(k)|\,|\,k\not\in\fml{F}_{\mbb{A}(\fml{E})}\}$
and $v_j = \min\{|\sv(k)|\,|\,k\in\fml{F}_{\mbb{A}(\fml{E})}\}$.
We plot $v_i$ in yellow and $v_j$ in blue, these pairs of values are depicted in \cref{fig:shap_scores}.
%
Another observation is that for the DT in~\cref{fig:dt03}, there are more than 151 out of 768 number of instances
exhibit this issue.
For the DT in~\cref{fig:dt04}, there are 82 out of 486 number of instances exhibit this issue.

Moreover, for the DT in~\cref{fig:dt03}, we found that
for the instance $((1, 0, 0, 0, 0, 0, 1, 1, 1), 1)$,
we have two AXps: $\{1, 5\}$ and $\{1, 4\}$
and the Sv of features are: $\sv(1)=0.3572$, $\sv(2)=-0.1428$, $\sv(3)=-0.0178$,
$\sv(4)=0.0449$, $\sv(5)=0.0449$, $\sv(6)=-0.0029$, $\sv(7)=-0.002$, $\sv(8)=0.0005$, $\sv(9)=0.0005$.
For this instance, feature 2 is irrelevant and feature 3 and 4 are relevant.
However, we have $|\sv(2)| > |\sv(3)|$ and $|\sv(2)| > |\sv(4)|$.
%
Additionally, for the same DT, we found two instances such that relevant features assigned with 0 Sv.
Specifically, for the instance $((1, 1, 1, 0, 2, 1, 1, 0, 1), 1)$, we can compute four AXps: $\{2\}$, $\{1, 5, 6, 7\}$, $\{1, 4\}$, and $\{1, 3\}$.
The Sv of features are: $\sv(1)=0.1172$, $\sv(2)=0.1373$, $\sv(3)=0.0123$, $\sv(4)=0.0123$,
$\sv(5)=0$, $\sv(6)=0.0016$, $\sv(7)=0.0016$, $\sv(8)=-0.0003$, $\sv(9)=0.0004$.
Clearly, feature 5 is relevant but its Sv is 0.
%
For another instance $((1, 1, 1, 0, 2, 1, 1, 1, 0), 1)$, we can compute four AXps: $\{2\}$, $\{1, 5, 6, 7\}$, $\{1, 4\}$, and $\{1, 3\}$.
The Sv of features are: $\sv(1)=0.1172$, $\sv(2)=0.1373$, $\sv(3)=0.0123$, $\sv(4)=0.0123$,
$\sv(5)=0$, $\sv(6)=0.0016$, $\sv(7)=0.0016$, $\sv(8)=0.0004$, $\sv(9)=-0.0003$.
Clearly, for the relevant feature 5, it has 0 Sv.



==> runex01.tex <==

\begin{figure}[t]
  \begin{subfigure}{0.65\linewidth}
    \scalebox{0.9725}{\input{./texfigs/tree01}}
    \caption{Decision tree}
  \end{subfigure}
  %
  \begin{subfigure}[c]{0.325\linewidth}
    \begin{minipage}{1.0\textwidth}
      \vspace*{0.45cm}\hspace*{-0.125cm}
      \scalebox{0.775}{
        \renewcommand{\arraystretch}{1.0}
        \renewcommand{\tabcolsep}{0.2175em}
        \begin{tabular}{ccc} \toprule
          \# & Name & Definition \\ \toprule
          1 & $A$ & $\tn{Age}>5$? \\ \midrule
          2 & $P$ & Petechiae? \\ \midrule
          3 & $N$ & Stiff Neck? \\ \midrule
          4 & $V$ & Vomiting? \\ \midrule
          5 & $Z$ & Zone${=}0,1,2$? \\ \midrule
          6 & $S$ & Seizures? \\ \midrule
          7 & $G$ & Gender? \\ \midrule
          8 & $H$ & Headache? \\ \midrule
          9 & $C$ & Coma? \\
          \bottomrule
          %\\%%[0.15cm]
        \end{tabular}
      }
    \end{minipage}
    \caption{Features'~meaning}
  \end{subfigure}
  \caption{First example DT, adapted from~\cite{belmonte-ieee-access20}} \label{fig:runex1}
\end{figure}


==> texfigs/dt00old.tex <==
% Concocted example
%%
%\tikzset{every label/.style={xshift=-0.35ex,
%  yshift=-5.25ex,
%  text width=1ex,
%  align=right, inner sep=1pt, font=\tiny, text=midblue}}
%%
%\tikzset{tlabel/.style={xshift=0.25ex, yshift=1.75ex, text width=1ex,
%    align=right, inner sep=1pt, font=\tiny, text=midblue}}
%%%\tikzset{every node/.style={---rectangle---}}
%
\forestset{
  BDT/.style={
    for tree={
      l=1.5cm,s sep=1.15cm,
      if n children=0{}{circle}, %rectangle
      %if n children=0{}{draw},
      draw=midblue,%draw=black,%
      text=midblue,%text=black,%
      edge={
        my edge
      },
      %if n=1{
      %  edge+={0 my edge},
      %}{},
      edge=thick,
      %font=\sffamily,
    }
  },
}
%
\begin{forest}
  BDT
  [{$x_1$}, label={[yshift=-6.875ex]{{\tiny1}}} 
    [{$x_2$}, label={[yshift=-6.875ex]{{\tiny2}}}, %edge={very thick}, %top-left=x
      edge label={node[midway,left,xshift=-0.5pt] {{\scriptsize$\in\{0\}$}}}
      [\dghlight{\textbf{4}}, label={[yshift=-5.25ex]{{\tiny8}}},
        edge label={node[midway,left,xshift=0.5pt] {{\scriptsize$\in\{0\}$}}}, rectangle, fill={tblue2!25} ]
      %
      [\dghlight{\textbf{0}}, label={[yshift=-5.25ex]{{\tiny5}}},
        edge label={node[midway,right,xshift=-0.5pt] {{\scriptsize$\in\{1\}$}}},
        rectangle, fill={tblue2!20} ]
    ]
    [\dghlight{\textbf{1}}, label={[yshift=-5.25ex]{{\tiny3}}},
      edge={very thick}, edge label={node[midway,right,xshift=0.5pt] {{\scriptsize$\in\{1\}$}}}, rectangle, fill={tblue2!25} ]
  ]
\end{forest}


==> tpl.tex <==

\subsection{Some Example -- Template}

\jnote{Template for presenting each example.}

\paragraph{Classifier.}
~\\

\paragraph{Feature influence on predicted class.}
~\\

\paragraph{Formal explanations \& feature relevancy.}
~\\

\paragraph{Features in adversarial examples.}
~\\

\paragraph{Shapley values \& feature importance.}
~\\

\paragraph{Instantiation -- If Applicable.}
~\\

\paragraph{Assessment.}
~\\


